Cross-Image Region Mining with Region Prototypical Network for Weakly Supervised Segmentation

Weakly supervised image segmentation trained with image-level labels usually suffers from inaccurate coverage of object areas during the generation of the pseudo groundtruth. This is because the object activation maps are trained with the classification objective and lack the ability to generalize. To improve the generality of the objective activation maps, we propose a region prototypical network RPNet to explore the cross-image object diversity of the training set. Similar object parts across images are identified via region feature comparison. Object confidence is propagated between regions to discover new object areas while background regions are suppressed. Experiments show that the proposed method generates more complete and accurate pseudo object masks, while achieving state-of-the-art performance on PASCAL VOC 2012 and MS COCO. In addition, we investigate the robustness of the proposed method on reduced training sets.

==> Figures/discover.tex <==
 \begin{figure*}[t]
 \centering
    \includegraphics[width=1\linewidth,height=0.3\linewidth]{Images/discover.pdf}
    \caption{The objects of the same category will activate different regions as object activate regions
    }
    \label{Figure:motivation}
\vspace{+0.3cm}
\end{figure*}

==> Figures/figure_cams.tex <==
 \begin{figure*}[t]
    \includegraphics[width=1\linewidth]{Images/cams.pdf}
    \caption{Visualization examples that compare the object active maps generated by our method with the object active maps generated by baseline methods. Our method can effectively expand object regions that are closer to the ground truth object regions. }
    \label{Figure:cams}
\vspace{+0.3cm}
\end{figure*}

==> Tables/combine_table.tex <==
\begin{table}[t]
\parbox{.45\linewidth}{
\centering

\caption{Comparison different features combination.}

\begin{tabular}{cc}
\toprule

method              & mIoU \\ \hline
baseline           & 49.1 \\
w/o cross-image relations & 49.8 \\
w/ cross-image relations & 50.8 \\  
\bottomrule

\end{tabular}
% \vskip +1em
\caption{The effectiveness of the cross-image relations between image pairs. Baseline is the basic network without our region prototype vector enhancement.}
\label{Table:two-way}
}

\hfill
\parbox{.45\linewidth}{
\centering
\begin{tabular}{cccc}
\toprule
block2 & block3 & block4 & mIoU      \\ \hline
\checkmark      &        &        & 50.0    \\
       & \checkmark      &        & 50.4  \\
       &        & \checkmark      & 50.1  \\
\checkmark      & \checkmark      &        & 48.8 \\
\checkmark      &        & \checkmark      & \textbf{50.8}  \\
       & \checkmark      & \checkmark      & 50.1 \\
\checkmark      & \checkmark      & \checkmark      & 50.4   \\
\bottomrule
\end{tabular}

\label{Table:feature-comparison}
}
\end{table}

==> Tables/combine_table_2.tex <==
\begin{table}[t]
\parbox{.65\linewidth}{
\centering
\caption{Comparison the performances of different probability to discard the object activation regions.}

\begin{tabular}{cccccc}
\toprule
Backbone           & Enhanced &Base  & Parameter & Top 1 error  \\ \hline
resnet50           & 49.8 &48.3 & 25.5M     & 23.8              \\
resnet101          & 51.0 &49.7 & 44.5M     & 22.6            \\
wide\_resnet50\_2  & 49.7 &48.4 & 68.9M     & 21.4              \\
wide\_resnet101\_2 & 50.8 &49.6 & 126.9M    & 21.1             \\
resnext\_50        & 50.8 &49.1 & 25.0M     & 22.3           \\
resnext\_101       & 52.8 &50.4 & 44.3M     & 20.6       \\

\bottomrule

\end{tabular}
\caption{Comparison different backbone performances. Base denotes the basic features without our RPNet . Enhanced denotes the features enhanced by our RPNet}

\label{Table:backbone}
}
\hfill
\parbox{.25\linewidth}{
\centering
\begin{tabular}{cc}
\toprule
Probability & mIoU   \\ \hline
0           & 49.8  \\
0.1         & 50.1   \\
0.3         & 50.2   \\
0.5         & 50.8   \\
0.7         & 50.5 \\
0.9         & 50.3  \\    
\bottomrule

\end{tabular}


\label{Table:hyper-parameter}
}
\vspace{+0.2cm}
\end{table}

==> Tables/compare_soa_combine_bk.tex <==
\begin{table*}[t]
\parbox{1\linewidth}{
\centering

\caption{Comparison of the weakly supervised semantic segmentation methods on PASCAL VOC 2012. Our method outperforms all the previous methods on both the validation set and the test set. WV denotes Web Video, S denotes Saliency Mask, WI denotes Web Image, IS denotes Instance Image. To be noted, our method outperforms all the previous methods with additional training data while we do not use any additional supervision.}

  \begin{tabular}{l|c|c|ccc}
  \toprule
    Method & AS & Val & Test\\
          \hline
      FCN-MIL~\cite{Pathak215}\tiny{ICLR2015}  &-  &  25.7 & 24.9 \\
      CCNN~\cite{Pathak15}\tiny{ICCV2015} &-   &  35.3 &35.6 \\
      EM-Adapt~\cite{papa15}\tiny{ICCV2015}  &-     &  38.2 &39.6 \\
      DCSM~\cite{dcsm}\tiny{ECCV2016}   &-   &  44.1 &45.1 \\
      BFBP~\cite{bfb}\tiny{ECCV2016} &-  &  46.6   &  48.0 \\
       SEC~\cite{sec}\tiny{ECCV2016}  &- &  50.7 &51.7 \\
      CBTS~\cite{cbts}\tiny{CVPR2017}  &-   &  52.8 &53.7 \\
      TPL~\cite{tphase}\tiny{ICCV2017} &- &  53.1 &53.8 \\
      MEFF~\cite{meff}\tiny{CVPR2018} &- &  - &55.6 \\
       PSA~\cite{psa}\tiny{CVPR2018}  &-   &  61.7 &63.7 \\
       IRN~\cite{irn}\tiny{CVPR2019} &- & 63.5 & 64.8 \\ 
       OAA+~\cite{oaa}\tiny{ICCV2019} &- & 65.2 & 66.4 \\ 
       SSDD~\cite{ssdd}\tiny{ICCV2019} &- & 64.9 &  65.5 \\
       CIAN~\cite{cian}\tiny{AAAI2020} &- & 62.4 &  65.3 \\
       MCI~\cite{mining-cross}\tiny{ECCV2020} &- & 66.2 &  66.9 \\
       SEAM~\cite{seam}\tiny{CVPR2020} &- & 64.5 &  65.7 \\
       BENet~\cite{benet}\tiny{ECCV2020} &- & 65.7 &  66.6 \\
        CONTA~\cite{conta}\tiny{NIPS2020}  &- & 65.3 &  66.1 \\
        \hline
        \hline
      MDC~\cite{mdc}\tiny{CVPR2018}       & S & 60.4 & 60.8 \\
      MCOF~\cite{mcof}\tiny{CVPR2018}    & S & 60.3 &61.2 \\
      DSRG~\cite{dsrg}\tiny{CVPR2018}   & S & 61.4 &63.2 \\
      Shen et al.~\cite{cvpr18web}\tiny{CVPR2018}   & WI  &  63.0 & 63.9 \\
      SeeNet~\cite{seenet}\tiny{NIPS2018}   & S & 63.1 &62.8 \\
       AISI~\cite{salins}\tiny{ECCV2018}      & IS & 63.6 &64.5 \\
       FickleNet~\cite{ficklenet}\tiny{CVPR2019} & S & 64.9 & 65.3 \\ 
       DSRG+EP.~\cite{DSRGEP}\tiny{ICCV2019} & S & 61.5 & 62.7 \\ 
      Zeng et al.~\cite{zeng_iccv2019} & S & 63.3 & 64.3 \\ 
      OAA+~\cite{oaa}\tiny{ICCV2019} & S & 65.2 & 66.4 \\ 
      SPM~\cite{spm}\tiny{ECCV2020} & S & 66.6 & 66.7 \\ 
       \hline
       
\textbf{RPNet} \tiny{(Resnet-50 w/o CRF)}      & -         & \textbf{65.1} & \textbf{66.0} \\ 

\textbf{RPNet} \tiny{(Resnet-50)}        & -         & \textbf{66.4} & \textbf{67.2} \\ 

    \textbf{RPNet} \tiny{(Resnext-50 w/o CRF)}       & -         & \textbf{65.7} & \textbf{66.7} \\ 

    \textbf{RPNet} \tiny{(Resnext-50) }       & -         & \textbf{67.0} & \textbf{68.1} \\ 
    
         \textbf{RPNet} \tiny{(Resnext-101 w/o CRF)}        & -  & \textbf{66.3} & \textbf{66.0} \\
         
     \textbf{RPNet}\tiny{ (Resnext-101) }      & -  & \textbf{68.0} & \textbf{68.2} \\ 
              \bottomrule
              
  \end{tabular}

\label{Table:comapre-soa-no-ad}
}
\vspace{+0.2cm}
\end{table*}
